Constrained clustering via diagrams: A unified theory and its applications to electoral district design

The paper develops a general framework for constrained clustering which is based on the close connection of geometric clustering and diagrams. Various new structural and algorithmic results are proved (and known results generalized and unified) which show that the approach is computationally efficient and flexible enough to pursue various conflicting demands. The strength of the model is also demonstrated practically on real-world instances of the electoral district design problem where municipalities of a state have to be grouped into districts of nearly equal population while obeying certain politically motivated requirements.

==> include/figures.tex <==
% set up externalization
\usetikzlibrary{external}



\tikzexternalize[shell escape=-enable-write18] % in windows: Tex-Live and MikTeX uses a -enable-write18 instead of --shell-escape.


\tikzsetexternalprefix{imgs/pgfexp/}
\tikzsetfigurename{figure}
\tikzset{external/force remake}

% uncomment for testing (nonexport)
%\tikzexternaldisable


%%%
%%enable for raster export and delete raster export properties below!!!
%%%%
 \tikzset{
	% % Defines a custom style which generates BOTH, .pdf and .png export
	% % but prefers the .png on inclusion.
	% %
	% % This style is not pre-defined, you may need to copy-paste and
	% % adjust it.
	raster export/.style={
		/pgf/images/external info,
		external/system call = {pdflatex
			\tikzexternalcheckshellescape -halt-on-error -interaction=batchmode -jobname
			"\image" "\texsource" && % or ;
			pdftops "\image".pdf
			&& convert -quality 100 -density 400 -colorspace cmyk -transparent white "\image.pdf"
			"\image.jpg"
		%	&& echo "\\includegraphics[width=/pgf/images/external/width,height=]" >>  figexpcode.tex
			 %			 echo "\includegraphics [width=\pgfexternalwidth,height=\pgfexternalheight]	{\image.jpg}" 
%			 echo "\includegraphics [width=\pgfexternalwidth,height=\pgfexternalheight]	{\image.jpg}" > figexpcode.tex%
			},
			/pgf/images/external info,
	%	/pgf/images/include external/.code={%
	%		\includegraphics
	%		[width=\pgfexternalwidth,height=\pgfexternalheight]
	%		{##1.jpg}%
		},
	%	}
		% %\pgfexternalheight
		% % /pgf/images/external info,
		% % /pgf/images/include external/.code={%
		% % \includegraphics
		% % [width=\pgfexternalwidth,height=\pgfexternalheight]
		% % {##1.png}%
		% % },
}

\tikzset{
	% % Defines a custom style which generates BOTH, .pdf and .png export
	% % but prefers the .png on inclusion.
	% %
	% % This style is not pre-defined, you may need to copy-paste and
	% % adjust it.
	vector export/.style={
		external/system call = {pdflatex
			\tikzexternalcheckshellescape -halt-on-error -interaction=batchmode -jobname
			"\image" "\texsource" && % or ;
			pdftops "\image".pdf
		}
		% %
		% % /pgf/images/external info,
		% % /pgf/images/include external/.code={%
		% % \includegraphics
		% % [width=\pgfexternalwidth,height=\pgfexternalheight]
		% % {##1.png}%
		% % },
}}

%
%\tikzset{
%	% % Defines a custom style which generates BOTH, .pdf and .png export
%	% % but prefers the .png on inclusion.
%	% %
%	% % This style is not pre-defined, you may need to copy-paste and
%	% % adjust it.
%	raster export/.style={
%		external/system call = {pdflatex
%			\tikzexternalcheckshellescape -halt-on-error -interaction=batchmode -jobname
%			"\image" "\texsource" && % or ;
%			pdftops "\image".pdf
%		}
%		% %
%		% % /pgf/images/external info,
%		% % /pgf/images/include external/.code={%
%		% % \includegraphics
%		% % [width=\pgfexternalwidth,height=\pgfexternalheight]
%		% % {##1.png}%
%		% % },
%}}

\newcommand{\imagefolderLQ}{imgs/raster300/}
\newcommand{\imagefolderHQ}{imgs/raster600/}
\newcommand{\imagefolder}{\imagefolderLQ}
% images

%% 
% 1:	Shortest Path WK13scale Clusters
%2:	Shortest Path WK13scale Abweichung Bund
%3:	Centroidal PD corrected Clustering
%4:	Centroidal PD corrected Abweichungen Bundesebene
%5:	wahlkreise2013 Clustering
%6:	wahlkreise2013 Abweichungen Bundesebene
%7:	wahlkreise2013 Abweichungen Landesebene
%8:	Shortest Path Clusters
%9:	Shortest Path Abweichung Bund
%10:	Laender
%11:	Bund Abweichunge nur über 15%
%12:	APD corrected Clusters
%13:	APD corrected Abweichung Bund
\newcommand{\bundPDFpage}[2]{\node[node distance=0, anchor=center] at
	(0,0) {\includegraphics[page=#1,width=#2,clip=false, trim=1.5cm 3.5cm
		1.3cm 2cm,]{\imagefolder bund.pdf}};} %hallo



%1:	Wahllreise 2013 Clustering
%2:	Wahllreise 2013 Abweichung Bundesebene
%3:	Centroidal PD Clustering
%4:	Centroidal PD Abweichung Bundesebene
%5:	CPD corrected Clustering
%6:	CPD corrected Abweichung Bundesebene
%7:	CPD clustering  power diagramm
%8:	Centroidal PD Sites
%9:	map
%10:	centroids
%11:	Shortest Path Clustering
%12:	Shortest Path Sites
%13:	Shortest Path Abweichung Bundesebene
%14:	Shortest Path Tree
%15:	CPD corrected fixed etc units
%16:	APD c13 BKM Corrected Clustering
%17:	APD c13 BKM Corrected Abweichung Bundesebene
%18:	APD c13 BKM Corrected Ellipsen
%19:	Landesgrenze
\newcommand{\bayernPDFpage}[1]{\node(img)[node distance=0, anchor=center] at
	(0,0) {\includegraphics[page=#1,width=\textwidth,clip=false, trim=0.7cm 0.5cm
		0.7cm 0.5cm,]{\imagefolder bayern.pdf}};}

%\newcommand{\bayernPDFpageIM}[3]{\node[node distance=0, anchor=center, #3] at
%	(0,0) {\includegraphics[page=#1,width=#2\textwidth,clip=false, trim=0.7cm 0.5cm
%		0.7cm 0.5cm,]{\imagefolderHQ bayern.pdf}};}

%  Lower Saxony APD - CPD - WK13 - SP
% 1:	Abweichung Bund Wahlen2013
% 2:	Abweichung Bund CPD corrected
% 3:	Abweichung Bund APD corrected
% 4:	Clustering Wahlkreise2013
% 5:	Clustering CPD corrected
% 6:	Clustering APD corrected
% 7:	Clustering PowerDiagram
% 8:	Clustering APD Ellipsen
% 9:	Clustering Shortest Path
% 10:	Abweichung Bund ShortestPath
% 11:	Shortest Path Tree
% 12:	Landesgrenze
% 13:	APD c13 bkm post FIxedUnits
\newcommand{\niedersachsenexmplPDFpage}[1]{\node(img)[node distance=0,
	anchor=center] at (0,0) {\includegraphics[page=#1,width=\textwidth,clip=false,
		trim=0.3cm 1.3cm 0.3cm 0.7cm]{\imagefolder niedersachsen.pdf}};}


%\newcommand{\niedersachsenexmplPDFpageIM}[3]{\node[node distance=0,
%	anchor=center, #3] at (0,0) {\includegraphics[page=#1,
%		width=#2\textwidth,clip=false, trim=0.3cm 1.3cm 0.3cm 0.7cm,]{\imagefolderHQ niedersachsen.pdf}};}
%


% Hesse
%1:	Wahllreise 2013 Clustering
%2:	Wahllreise 2013 Abweichung Bundesebene
%3:	Centroidal PD Clustering
%4:	Centroidal PD Abweichung Bundesebene
%5:	CPD corrected Clustering
%6:	CPD corrected Abweichung Bundesebene
%7:	CPD clustering  power diagramm
%8:	Centroidal PD Sites
%9:	map
%10:	centroids
%11:	Shortest Path Clustering
%12:	Shortest Path Sites
%13:	Shortest Path Abweichung Bundesebene
%14:	Shortest Path Tree
%15:	CPD corrected fixed etc units
%16:	APD c13 BKM Corrected Clustering
%17:	APD c13 BKM Corrected Abweichung Bundesebene
%18:	APD c13 BKM Corrected Ellipsen
%19:	Landesgrenze
\newcommand{\hessenexmplPDFpage}[1]{\node(img)[node distance=0,
	anchor=center] at (0,0)
	{\includegraphics[page=#1,width=.95\textwidth,clip=false, trim=0.3cm 0.6cm 0.3cm
		0.2cm]{\imagefolder hessen.pdf}};}


%% NRW
%1:	Wahllreise 2013 Clustering
%2:	Wahllreise 2013 Abweichung Bundesebene
%3:	Centroidal PD Clustering
%4:	Centroidal PD Abweichung Bundesebene
%5:	CPD corrected Clustering
%6:	CPD corrected Abweichung Bundesebene
%7:	CPD clustering  power diagramm
%8:	Centroidal PD Sites
%9:	map
%10:	centroids
%11:	Shortest Path Clustering
%12:	Shortest Path Sites
%13:	Shortest Path Abweichung Bundesebene
%14:	Shortest Path Tree
%15:	CPD corrected fixed etc units
%16:	APD c13 BKM Corrected Clustering
%17:	APD c13 BKM Corrected Abweichung Bundesebene
%18:	APD c13 BKM Corrected Ellipsen
%19:	Landesgrenze

\newcommand{\nrwexmplPDFpage}[1]{\node(img)[node distance=0,
	anchor=center] at (0,0)
	{\includegraphics[page=#1,width=.95\textwidth,clip=false, trim=0.3cm 0.3cm 0.3cm
		0.2cm]{\imagefolder nordrheinwestfalen.pdf}};}




\tikzset{
	unit/.style={circle,fill=TUMhighlight, draw=TUMdarkblue, minimum size = 10pt,
		line width = 2pt, node distance = 2cm},
	site/.style={draw,rectangle, black, line width = 3pt ,fill=white, minimum size =
		10pt, node distance = 2cm},
	path/.style={decorate, decoration={snake,segment length=4mm,post
			length=1mm}}, edge/.style={bend left = 20},
	wlabel/.style={black!70,below=5pt},
	legendmarker/.style={rectangle,draw=black!70, line width = 1pt, minimum width
		= 0.7cm, minimum height = 0.4cm, node distance = .6cm},
	legendlabel/.style={right=.4cm} }

\definecolor{devcolor5}{RGB}{26,150,65}
\definecolor{devcolor15}{RGB}{220,255,196}
\definecolor{devcolor25}{RGB}{253,105,0}
\definecolor{devcolor100}{RGB}{215,25,0}


 \newcommand{\figureDevGermanyElection}{
 	\tikzsetnextfilename{fig01a}
 	 \bgroup
\tikzset{raster export}
 \begin{tikzpicture}
  \bundPDFpage{6}{\textwidth} % Abweichung 2013
 \end{tikzpicture}
 \egroup
}
 
 
  \newcommand{\figureDevGermanySP}{
  	\tikzsetnextfilename{fig01b}
 \bgroup
 \tikzset{raster export}
  \begin{tikzpicture}
   \bundPDFpage{9}{\textwidth} % Abweichung shortest Pth
 \end{tikzpicture}
 \egroup
 }
 

  
  \newcommand{\legendlabel}[3]{
    \begin{tabular}{R{.2cm}@{}R{.8cm}@{}R{1.1cm}@{}}
    	#1 & #2 & #3
    \end{tabular}
 }
  \newcommand{\figureDevLegend}{
  	\tikzsetnextfilename{fig01c}
  	\bgroup
  	\tikzset{vector export}
 % \hfill
% \raisebox{45mm}[0mm][0mm]{
%\fbox{
 	\begin{tikzpicture}
 		 
 		 \useasboundingbox (-.5cm,-1cm) rectangle (3.3cm,5.5cm);
 		 
 		  \node(lm1)[legendmarker, fill = devcolor5] at (0.5cm,3.6cm) {};
 		  \node(ll1) [legendlabel, right of=lm1] {\legendlabel{$\big[$}{$0\%,$}{$5\%\big]$}};
 		  
 		  \node(lm2)[legendmarker, fill = devcolor15, below of=lm1] {};
 		  \node(ll2) [legendlabel, right of=lm2] {\legendlabel{$\big($}{$5\%,$}{$15\%\big]$}};
 		  
 		  \node(lm3)[legendmarker, fill = devcolor25, below of=lm2] {};
 		  \node(ll3) [legendlabel, right of=lm3] {\legendlabel{$\big($}{$15\%,$}{$25\%\big]$}};
 		  
 		  
 		  \node(lm4)[legendmarker, fill = devcolor100, below of=lm3] {};
 		  \node(ll4) [legendlabel, right of=lm4] {\legendlabel{$\big($}{$25\%,$}{$100\%\big]$}};
 		  
 		  
 	\end{tikzpicture}
%}	
% 	
% \hspace{-2pt}\begin{tabular}{m{.7cm}r@{}r@{\hspace{.2em}}r@{}}
% %& \multicolumn{3}{c}{Deviation} \\
% %\vspace{4pt}
%  \begin{tikzpicture}
%  \node[legendmarker, fill = devcolor5] {};
%  \end{tikzpicture}&   $\big[$&$0\%,$&$5\%\big]$ \\
%% \hline 
% %\vspace{4pt}
% \begin{tikzpicture}
% \node[legendmarker, fill = devcolor15] {};
% \end{tikzpicture} & $\big($&$5\%,$&$15\%\big]$ \\
%% \hline 
%%\vspace{4pt}
%\begin{tikzpicture}
% \node[legendmarker, fill = devcolor25] {};
% \end{tikzpicture} & $\big($&$15\%,$&$25\%\big]$  \\
%% \hline 
%% \vspace{4pt}
%\begin{tikzpicture}
% \node[legendmarker, fill = devcolor100] {};
% \end{tikzpicture} & $\big($&$25\%,$&$100\%\big]$ 
% \end{tabular}
%}
\egroup
}

\newcommand{\figureExampleOnlyAffineTrans}{
	\tikzsetnextfilename{fig10}
	\bgroup
	\tikzset{vector export}
\begin{tikzpicture}


\node(s1)[site, label=below:{$x_1 = s_1$}] {};

\node(x2)[unit,
label=below:$\unit_2$] [right of = s1]{};

\node(x3)[unit, label=right:$\unit_3$] [above of =x2] {};


\node(s2)[site, label=below:{$\unit_4 = s_2$}] [right of =x2] {};

\draw[edge] (s1)  --  node[above] {$a$} (x2) ;
\draw[edge] (x2) -- node[right] {$b$}  (x3);
\draw[edge] (x2) -- node[above] {$c$} (s2);

\end{tikzpicture}
\egroup
}

\newcommand{\figureZoomedClusteringFracts}{
	\tikzsetnextfilename{fig11}
	\bgroup
	\tikzset{vector export}
\begin{tikzpicture}[zoomboxarray,zoomboxarray inner gap=0.5cm, zoomboxarray
columns=1, zoomboxarray rows=1, connect zoomboxes,  zoombox paths/.append
style={ultra thick, black}] \node[image node] {\includegraphics[width =
	0.22\textwidth]{imgs/08GraphClusteringfracts}};
\zoombox[magnification=4.3,color code=black]{.55,0.5}
\end{tikzpicture}
\egroup
}


\newcommand{\figureZoomedClusterinSquaredConnected}{
	\tikzsetnextfilename{fig12}
	\bgroup
	\tikzset{vector export}
\begin{tikzpicture}[zoomboxarray,zoomboxarray inner gap=0.5cm, zoomboxarray
columns=1, zoomboxarray rows=1, connect zoomboxes,  zoombox paths/.append
style={ultra thick, black}] \node[image node] {\includegraphics[width =
	0.22\textwidth]{imgs/09GraphClusteringSquarednonconnected}};
\zoombox[magnification=8,color code=black]{.34,0.83}
\end{tikzpicture}
\egroup
}


\newcommand{\figureBayernOriginalDistricts}{
		\tikzsetnextfilename{fig13a}
\bgroup
	\tikzset{raster export}
\begin{tikzpicture}
\bayernPDFpage{19} 
\bayernPDFpage{1} 
\end{tikzpicture}
\egroup
}

\newcommand{\figureBayernPowerDiagram}{
	\tikzsetnextfilename{fig13b}
	\bgroup
	\tikzset{raster export}
 \begin{tikzpicture}
 \bayernPDFpage{19} 
\bayernPDFpage{5} % Clustering CPD
% \bayernPDFpage{18} 
\bayernPDFpage{7} % Clustering CPD
\end{tikzpicture}
\egroup
}

\newcommand{\figureNiedersachsenOriginalDistricts}{
		\tikzsetnextfilename{fig14a}
	\bgroup
	\tikzset{raster export}
 \begin{tikzpicture}
 \niedersachsenexmplPDFpage{19}
\niedersachsenexmplPDFpage{1} % Clustering 13
\end{tikzpicture}
\egroup
}

\newcommand{\figureNiedersachsenAPD}{
		\tikzsetnextfilename{fig14b}
	\bgroup
	\tikzset{raster export}
 \begin{tikzpicture}
  \niedersachsenexmplPDFpage{19}
\niedersachsenexmplPDFpage{16} % Clustering APD
%\niedersachsenexmplPDFpage{13} % Clustering APD ellipsen
\niedersachsenexmplPDFpage{18} % Clustering APD
\end{tikzpicture}
\egroup
}

\newcommand{\figureNRWOriginalDistricts}{
		\tikzsetnextfilename{fig15a}
	\bgroup
	\tikzset{raster export}
\begin{tikzpicture}
\nrwexmplPDFpage{19} 
\nrwexmplPDFpage{1} % Clustering 13
\end{tikzpicture}
\egroup
}

\newcommand{\figureNRWSP}{
		\tikzsetnextfilename{fig15b}
	\bgroup
	\tikzset{raster export}
\begin{tikzpicture}
\nrwexmplPDFpage{19} 
\nrwexmplPDFpage{11} % Clustering APD
\nrwexmplPDFpage{14} % Clustering CPD
\end{tikzpicture}
 \egroup
}

\newcommand{\figureBundDevPD}{
		\tikzsetnextfilename{fig16a}
	\bgroup
	\tikzset{raster export}
\begin{tikzpicture}
\bundPDFpage{4}{\textwidth} % Abweichung Power Diagram
\end{tikzpicture}
\egroup
}

\newcommand{\figureBundDevAPD}{
	\tikzsetnextfilename{fig16b}
	\bgroup
	\tikzset{raster export}
\begin{tikzpicture}
\bundPDFpage{13}{\textwidth} % Abweichung Anistropic Power Diagram
\end{tikzpicture}
\egroup
}

\newcommand{\figureBundDevSP}{
	\tikzsetnextfilename{fig16c}
	\bgroup
	\tikzset{raster export}
 \begin{tikzpicture}
\bundPDFpage{9}{\textwidth} % Abweichung Shortest Path
\end{tikzpicture}
\egroup
}


\newcommand{\figureHessenOriginalDistricts}{
	\tikzsetnextfilename{fig17a}
	\bgroup
	\tikzset{raster export}
 \begin{tikzpicture}
  \hessenexmplPDFpage{19}
\hessenexmplPDFpage{1}
\end{tikzpicture}
\egroup
}

\newcommand{\figureHessenPD}{
	\tikzsetnextfilename{fig17b}
	\bgroup
	\tikzset{raster export}
 \begin{tikzpicture}
 \hessenexmplPDFpage{19}
\hessenexmplPDFpage{3}  % cpd clustering
%\hessenexmplPDFpage{13}  % fixed units
%\hessenexmplPDFpage{6} %power diagram
\end{tikzpicture}
\egroup
}

\newcommand{\figureHessenAPD}{
	\tikzsetnextfilename{fig17c}
	\bgroup
	\tikzset{raster export}
\begin{tikzpicture}
 \hessenexmplPDFpage{19}
\hessenexmplPDFpage{16} % apd clustering
%\hessenexmplPDFpage{12} % ellipsen
% \hessenexmplPDFpage{14}  % fixed units
\end{tikzpicture}
\egroup
}


\newcommand{\figureHessenSP}{
	\tikzsetnextfilename{fig17d}
	\bgroup
	\tikzset{raster export}
\begin{tikzpicture}
 \hessenexmplPDFpage{19}
\hessenexmplPDFpage{11} 
\end{tikzpicture}
\egroup
}


\newcommand{\figureToyEx}{
	\includegraphics[width = 0.43\textwidth]{imgs/01Instance}
}


\newcommand{\figureToyExAWVD}{
	\includegraphics[width = 0.43\textwidth]{imgs/02AwVoronoiDiagram}
}

\newcommand{\figureToyExPD}{
\includegraphics[width = 0.43\textwidth]{imgs/03PowerDiagram}
}

\newcommand{\figureToyExAVD}{
	\includegraphics[width =  0.43\textwidth]{imgs/04AnistropVoronoiDiagram}
}


\newcommand{\figureToyExAPD}{
	\includegraphics[width =  0.43 \textwidth]{imgs/05AnistropPowerDiagram}
}

\newcommand{\figureToyExSP}{
	\includegraphics[width = 0.43 \textwidth]{imgs/06GraphClustering}
}


\newcommand{\figureToyExSPSQ}{
	 \includegraphics[width =  0.43\textwidth]{imgs/07GraphClusteringSquared}
}

\newcommand{\figureToyExPDDiagram}{
	\includegraphics[width=\textwidth]{imgs/10PowerDiagramonlydiagram.pdf}
}

\newcommand{\figureToyExAPDDiagram}{
 \includegraphics[width=\textwidth]{imgs/11AnistropPowerDiagramonlydiagram.pdf}
}

\newcommand{\figureToyExSPDiagram}{
\includegraphics[width=\textwidth]{imgs/12GraphClusteringonlydiagram.pdf}
}

